SOAP: A generalised application of the Viterbi algorithm to searches for continuous gravitational-wave signals

All-sky and wide parameter space searches for continuous gravitational waves are generally template-matching schemes which test a bank of signal waveforms against data from a gravitational wave detector. Such searches can offer optimal sensitivity for a given computing cost and signal model, but are highly-tuned to specific signal types and are computationally expensive, even for semi-coherent searches. We have developed a search method based on the well-known Viterbi algorithm which is model-agnostic and has a computational cost several orders of magnitude lower than template methods, with a modest reduction in sensitivity. In particular, this method can search for signals which have an unknown frequency evolution. We test the algorithm on three simulated and real data sets: gapless Gaussian noise, Gaussian noise with gaps and real data from the final run of initial LIGO (S6). We show that at 95% efficiency, with a 1% false alarm rate, the algorithm has a depth sensitivity of $\sim 33$, $10$ and $13$ ,Hz$^{-1/2}$ with corresponding SNRs of $\sim 60$, $72$ and $74$ in these datasets. we discuss the use of this algorithm for detecting a wide range of quasi-monochromatic gravitational wave signals and instrumental lines.

==> Makefile <==
DOCS = soap.pdf

FIGS = ./figures/s6_efficiency_depth.pdf \
./figures/s6_efficiency_snr.pdf \
./figures/viterbi_tracks.pdf \
./figures/gaussian_eff_snr.pdf \
./figures/gaussian_eff_depth.pdf \
./figures/gaussian_res_depth.pdf \
./figures/gaussian_res_snr.pdf \
./figures/gauss_s6_eff_depth.pdf \
./figures/gauss_s6_eff_snr.pdf \
./figures/gauss_s6_frac_depth.pdf \
./figures/gauss_s6_frac_snr.pdf \
./figures/vit_data.pdf \
./figures/vit_prob.pdf \


TABLES = 

BIBLIO = ./soap.bib

BYPROD = *.aux *.log *.out *.dvi *.bbl *.blg

default: git-tag $(DOCS) $(FIGS)

.PHONY : git-tag

git-tag:
	./git-tag.sh

soap.pdf: soap.tex $(FIGS) $(TABLES) $(BIBLIO)
	pdflatex $(@:.pdf=) && bibtex $(@:.pdf=) && pdflatex $(@:.pdf=) && pdflatex $(@:.pdf=) && pdflatex $(@:.pdf=)

%.pdf: %.eps
	epstopdf --outfile=$@ $(@:.pdf=.eps)

clean:
	rm -f $(DOCS) $(BYPROD)

